Efficient Monte Carlo Tree Search via On-the-Fly State-Conditioned Action Abstraction

Monte Carlo Tree Search (MCTS) has showcased its efficacy across a broad spectrum of decision-making problems. However, its performance often degrades under vast combinatorial action space, especially where an action is composed of multiple sub-actions. In this work, we propose an action abstraction based on the compositional structure between a state and sub-actions for improving the efficiency of MCTS under a factored action space. Our method learns a latent dynamics model with an auxiliary network that captures sub-actions relevant to the transition on the current state, which we call state-conditioned action abstraction. Notably, it infers such compositional relationships from high-dimensional observations without the known environment model. During the tree traversal, our method constructs the state-conditioned action abstraction for each node on-the-fly, reducing the search space by discarding the exploration of redundant sub-actions. Experimental results demonstrate the superior sample efficiency of our method compared to vanilla MuZero, which suffers from expansive action space.

==> table/action_space_reduction.tex <==
\begin{table}[t!]
\caption{Action space reduction.}
\label{table:action_space_reduction}
% \vspace{-5pt}
\centering
\begin{adjustbox}{width=0.48\textwidth}%\setlength{\tabcolsep}{4pt}
\begin{tabular}{cccccc}
\toprule
\multicolumn{3}{c}{\makecell{DoorKey}} & \multicolumn{3}{c}{\makecell{Sokoban}}\\
\cmidrule(lr){1-3}
\cmidrule(lr){4-6}

Easy& Normal& Hard& Easy& Normal& Hard\\
\midrule
66.7\% & 75.0\% & 80.0\% & 46.7\% & 88.9\% & 95.2\% \\
\bottomrule
\end{tabular}
\end{adjustbox}
% \vspace{-0.5cm}
\end{table}

==> table/training_time_comp.tex <==
\begin{table}[t!]
\caption{Training time comparison.}
\label{table:training_time}
% \vspace{-5pt}
\centering
\begin{adjustbox}{width=0.48\textwidth}%\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lcccccc}
\toprule
Models & 4h & 8h & 12h & 16h & 20h \\
\midrule
Ours & -116.39& -13.00 & -3.89 & -5.30 & -2.19 \\
MuZero & -134.16 & -114.96 & -80.60 & -52.21 & -49.60 \\
\bottomrule
\end{tabular}
\end{adjustbox}
% \vspace{-0.5cm}
\end{table}
